Eventually Consistent Register Revisited

In order to converge in the presence of concurrent updates, modern eventually consistent replication systems rely on causality information and operation semantics. It is relatively easy to use semantics of high-level operations on replicated data structures, such as sets, lists, etc. However, it is difficult to exploit semantics of operations on registers, which store opaque data. In existing register designs, concurrent writes are resolved either by the application, or by arbitrating them according to their timestamps. The former is complex and may require user intervention, whereas the latter causes arbitrary updates to be lost. In this work, we identify a register construction that generalizes existing ones by combining runtime causality ordering, to identify concurrent writes, with static data semantics, to resolve them. We propose a simple conflict resolution template based on an application-predefined order on the domain of values. It eliminates or reduces the number of conflicts that need to be resolved by the user or by an explicit application logic. We illustrate some variants of our approach with use cases, and how it generalizes existing designs.

==> mathdefs.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}

% macros for domain teory, semantics, etc. 

% math code definitions

%%%%%%%%%%%%%%%%%%%%%%%%\mathcode`:="603A          % : as punctuation
\mathcode`.="613A          % . as punctuation
\mathcode`|="326A          % | as a relation

\let\es=\relax    %  possible space before punctuation in displayed formulas

%% relations

\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\let\vect=\overrightarrow
\let\iff=\Leftrightarrow        % this redefines the original
%\let\implies=\Rightarrow
\let\implied=\Leftarrow

\let\sqleq=\sqsubseteq
\let\sqgeq=\sqsupseteq
\let\pleq=\sqleq          % partial-order leq
\let\pgeq=\sqgeq          % partial-order geq

\def\land{\mathrel{\wedge}}
\def\lor{\mathrel{\vee}}
\let\bigland=\bigwedge
\let\biglor=\bigvee

\def\preleq{\mathrel{%      % pre-order leq
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}

% operators

\let\union=\cup
\let\bigunion=\bigcup
\let\join=\sqcup
\let\bigjoin=\bigsqcup
\let\meet=\sqcap
%\let\bigmeet=\bigsqcap
\newcommand{\down}{\mathord{\downarrow}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
%\newcommand\domsub{\mathbin{\stackrel{-}{|}}}
\newcommand\domainsub{\mathop{\lhd\mkern-14mu-}}

% arrows

\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}

% function constants

\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
 \newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
 \newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}

\auxfun{Max}
\auxfun{fix}
\auxfun{dom}
\auxfun{fst}
\auxfun{snd}
\auxfun{ran}

% sets

\newcommand{\pow}[1]{{\cal P}(#1)}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\ids}{\mathds{I}}



%%%%%%%%%%%

\newcommand\letin[2]{\mathop{\hbox{$\mathrm{let}$}} #1 \Leftarrow #2 . }
\newcommand\lift[1]{\lfloor #1 \rfloor}

\newcommand\true{\mathrm{true}}
\newcommand\false{\mathrm{false}}

%%%%%%%%%%%%%%%%%%%%%

\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}
\newcommand\pfunc{\hookrightarrow}
\newcommand\func{\rightarrow}


